AMPED: Adaptive Multi-objective Projection for balancing Exploration and skill Diversification

Skill-based reinforcement learning (SBRL) enables rapid adaptation in environments with sparse rewards by pretraining a skill-conditioned policy. Effective skill learning requires jointly maximizing both exploration and skill diversity. However, existing methods often face challenges in simultaneously optimizing for these two conflicting objectives. In this work, we propose a new method, Adaptive Multi-objective Projection for balancing Exploration and skill Diversification (AMPED), which explicitly addresses both: during pre-training, a gradient-surgery projection balances the exploration and diversity gradients, and during fine-tuning, a skill selector exploits the learned diversity by choosing skills suited to downstream tasks. Our approach achieves performance that surpasses SBRL baselines across various benchmarks. Through an extensive ablation study, we identify the role of each component and demonstrate that each element in AMPED is contributing to performance. We further provide theoretical and empirical evidence that, with a greedy skill selector, greater skill diversity reduces fine-tuning sample complexity. These results highlight the importance of explicitly harmonizing exploration and diversity and demonstrate the effectiveness of AMPED in enabling robust and generalizable skill learning. Project Page: https://geonwoo.me/amped/

==> writings/main/Introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% Efficient exploration remains a major challenge in reinforcement learning (RL), particularly in environments with sparse or delayed rewards~\citep{sut-bart, biological1, biological2, biological3}. 
% In that case, agents often rely on handcrafted reward functions, which demand extensive domain knowledge and limit scalability~\citep{reward}. 
% Skill-Based RL (SBRL) addresses this by pretraining a skill-conditioned policy through unsupervised skill discovery~\citep{VIC, SkiMo}. % , enabling efficient adaptation to downstream tasks.

Efficient exploration remains a major challenge in reinforcement learning (RL), particularly in environments with sparse or delayed rewards~\citep{sut-bart, biological1, biological2, biological3}. While biological agents naturally discover rewarding behaviors, artificial agents often rely on handcrafted reward functions, which demand extensive domain knowledge and limit scalability~\citep{reward}. Skill-Based Reinforcement Learning (SBRL) addresses this by pretraining a skill-conditioned policy through unsupervised skill discovery~\citep{VIC, SkiMo}, enabling efficient adaptation to downstream tasks.


A common approach in SBRL is to use Unsupervised Reinforcement Learning (URL) objectives during pretraining to discover diverse and useful skills~\citep{DIAYN, VIC}.
Two widely used URL objectives are: (1) maximizing mutual information (MI) between skills and their state trajectories to promote skill diversity, and (2) maximizing state entropy to encourage exploration~\citep{CIC, APT} (Appendix~\ref{sec:appendix:related_works}).
However, MI-driven objectives often induce premature specialization by curtailing exploration~\citep{EDL,ReST, DISDAIN}, while entropy-based exploration sacrifices skill distinguishability, limiting downstream utility. 
The core problem is how to balance these competing objectives, without resorting to ad-hoc heuristics.

In this work, we bridge two URL paradigms in the theoretical framework of multi-objective reinforcement learning, proposing Adaptive Multi-objective Projection for balancing Exploration and skill Diversification (AMPED).
Few previous studies, such as CeSD~\citep{CeSD} and ComSD~\citep{ComSD}, have explored similar integrations but either lack a solid theoretical foundation or exhibit significant limitations (Appendix \ref{sec:appendix:difference_with_former_studies}).


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{main/scheme_a.pdf}
        \caption{Initialization}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{main/scheme_b.pdf}
        \caption{Maximization}
    \end{subfigure}
    \begin{tikzpicture}
        \draw[dashed, thick] (0,4.0) -- (0,9.0);
    \end{tikzpicture}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{main/scheme_c.pdf}
        \caption{Skill Selection}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\linewidth]{main/scheme_d.pdf}
        \caption{Adaptation}
    \end{subfigure}
    \caption{\textbf{Graphical scheme explaining our method, AMPED.}
(a) At initialization, the skills exhibit small coverage that are close to each other in the task space. 
(b) During skill pretraining, exploration and diversity objectives encourage skills to widen and repel each regions. 
(c) In fine-tuning, the skill selector identifies the skill best aligned with the target task at each step.
(d) The selected skill is further adapted via extrinsic rewards to maximize performance on the target task.}
    \vspace{-1.5em}
    \label{fig:amped_pipeline}
\end{figure}
Our key insight is that gradient conflicts naturally arise between diversity objectives and exploration objectives, leading to inefficient updates that hinder learning~\citep{gradient_conflict}. 
To address this issue, we adopt a gradient surgery method inspired by multi-objective RL, ensuring that conflicting gradient components are removed before applying updates~\citep{gradient_conflict}.  
We use particle-based entropy and Random Network Distillation (RND) \citep{RND} to drive exploration, and adopt the AnInfoNCE objective for skill diversity.
Furthermore, rather than selecting skills uniformly at random during fine‐tuning, as is common in prior SBRL approaches \citep{CeSD, DIAYN, BeCL}, we introduce a Soft Actor‐Critic (SAC) based skill selector that learns to select the best matching pretrained skill~\citep{SAC}. 
This adaptive selection manner maximally leverages the inherent diversity of the skill repertoire.
A graphical summary of these contributions is provided in Figure~\ref{fig:amped_pipeline}.

AMPED improves performance over strong baselines, DIAYN, COMSD, RND, CeSD, BeCL, CIC, and APT, across benchmarks. We evaluate AMPED on Maze environments~\citep{edl_github} and the Unsupervised Reinforcement Learning Benchmark (URLB)~\citep{URLB}. In the Maze suite, AMPED learns well-separated skills while simultaneously achieving high state coverage, whereas competing methods fail to maximize both.  
On URLB, AMPED achieves statistically well-supported and consistent improvements in return over the baselines, as measured using the robust evaluation protocol of \citet{DRL_Precipice}.
Taken together, these results show that explicitly resolving exploration-diversity gradient conflicts yields substantial gains in SBRL.

Ablation studies further confirm that each component of our framework, entropy bonuses, RND, Anisotropic InfoNCE, gradient surgery, and the skill selector, contributes meaningfully to overall performance. Moreover, we show, theoretically, that greater skill diversity reduces fine-tuning sample complexity when paired with a greedy skill selector. This clarifies the respective roles of diversity and selection and motivates further work on principled skill selector design.

\vspace{-0.5em}

% We provide the full implementation of AMPED to facilitate the reproduction of our main results at \textcolor{RoyalBlue}{\url{https://github.com/Cho-Geonwoo/amped}}.

% \vspace{-1em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section: Related work
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

